Towards Efficient Discrete Integration via Adaptive Quantile Queries

Discrete integration in a high dimensional space of n variables poses fundamental challenges. The WISH algorithm reduces the intractable discrete integration problem into n optimization queries subject to randomized constraints, obtaining a constant approximation guarantee. The optimization queries are expensive, which limits the applicability of WISH. We propose AdaWISH, which is able to obtain the same guarantee but accesses only a small subset of queries of WISH. For example, when the number of function values is bounded by a constant, AdaWISH issues only O(log n) queries. The key idea is to query adaptively, taking advantage of the shape of the weight function being integrated. In general, we prove that AdaWISH has a regret of only O(log n) relative to an idealistic oracle that issues queries at data-dependent optimal points. Experimentally, AdaWISH gives precise estimates for discrete integration problems, of the same quality as that of WISH and better than several competing approaches, on a variety of probabilistic inference benchmarks. At the same time, it saves substantially on the number of optimization queries compared to WISH. On a suite of UAI inference challenge benchmarks, it saves 81.5% of WISH queries while retaining the quality of results.

==> review.tex <==
Figure 1:
Change “The yellow and blue curves” to “The filled and dashed curves”, also remove color references.\\

Algorithm 1, line 5:
use $H_i^t$ instead of '$H_t$'.\\

Section 2:
add ‘for any $c\geq 2$’ before Lemma 2 for better understanding.\\

Typo errors:\\
Section 3.1:\\
Equations (1) and (2) - The $\phi$ symbols used for $\phi^E$ are inconsistent. Fixed.\\
"function SEARCH called" $\rightarrow$ "function SEARCH was called"\\
"technique report" $\rightarrow$ "technical report"\\

Section 4:
"minuets" $\rightarrow$ "minutes"\\

Q: Theorem 5 works assuming a deterministic algorithm.\\

A: changed corollary 1. and lower bound in introduction
\\
\\
meta review:
incorporate statements:
\begin{enumerate}
    \item the theory and guarantees are being developed in an oracle model that assumes a form of randomization in the oracle
    \item whether the randomization can be achieved in a practical oracle implementation is an open problem. but the theory stands on its own in that oracle model of computation.
    \item one can still develop an algorithm inspired by this randomized oracle theory that gives good results in practice, albeit without retaining the formal guarantees
\end{enumerate}

review 2:
cite SWITCH paper. 
\\https://link.springer.com/chapter/10.1007/978-3-030-30048-7$\_$10
